Generative Learning of Counterfactual for Synthetic Control Applications in Econometrics

A common statistical problem in econometrics is to estimate the impact of a treatment on a treated unit given a control sample with untreated outcomes. Here we develop a generative learning approach to this problem, learning the probability distribution of the data, which can be used for downstream tasks such as post-treatment counterfactual prediction and hypothesis testing. We use control samples to transform the data to a Gaussian and homoschedastic form and then perform Gaussian process analysis in Fourier space, evaluating the optimal Gaussian kernel via non-parametric power spectrum estimation. We combine this Gaussian prior with the data likelihood given by the pre-treatment data of the single unit, to obtain the synthetic prediction of the unit post-treatment, which minimizes the error variance of synthetic prediction. Given the generative model the minimum variance counterfactual is unique, and comes with an associated error covariance matrix. We extend this basic formalism to include correlations of primary variable with other covariates of interest. Given the probabilistic description of generative model we can compare synthetic data prediction with real data to address the question of whether the treatment had a statistically significant impact. For this purpose we develop a hypothesis testing approach and evaluate the Bayes factor. We apply the method to the well studied example of California (CA) tobacco sales tax of 1988. We also perform a placebo analysis using control states to validate our methodology. Our hypothesis testing method suggests 5.8:1 odds in favor of CA tobacco sales tax having an impact on the tobacco sales, a value that is at least three times higher than any of the 38 control states.

==> backup <==
@misc{sourceincome,
  title = {Per Capita Personal Income in California [CAPCPI]},
  howpublished = {\url{https://fred.stlouisfed.org/series/CAPCPI}},
  note = {U.S. Bureau of Economic Analysis, Per Capita Personal Income in California [CAPCPI], retrieved from FRED, Federal Reserve Bank of St. Louis; July 12, 2019.},
  year={}
}


@misc{sourcetobacco,
  title = {The Tax Burden on Tobacco 1970-2018},
  howpublished = {\url{https://chronicdata.cdc.gov/Policy/The-Tax-Burden-on-Tobacco-1970-2018/7nwe-3aj9}},
    year={}

}



@incollection{transforms,
 author = {{Zarembka} P.},
 year = {1990},
 title = {Transformation of Variables in Econometrics},
 editor = {Eatwell J. and Milgate M. and Newman P.},
 book = {Econometrics},
 publisher = {The New Palgrave. Palgrave Macmillan, London},
 doi = {https://doi.org/10.1007/978-1-349-20570-7_36}
}


@TechReport{Ferman16,
  author={Ferman, Bruno and Pinto, Cristine},
  title={{Revisiting the Synthetic Control Estimator}},
  year=2016,
  month=Sep,
  institution={University Library of Munich, Germany},
  type={MPRA Paper},
  url={https://ideas.repec.org/p/pra/mprapa/73982.html},
  number={73982},
  abstract={},
  keywords={synthetic control; difference-in-differences; linear factor model; inference; permutation test},
  doi={},
}




@techreport{synetheticdid,
 title = "Synthetic Difference In Differences",
 author = "Arkhangelsky, Dmitry and Athey, Susan and Hirshberg, David A and Imbens, Guido W and Wager, Stefan",
 institution = "National Bureau of Economic Research",
 type = "Working Paper",
 series = "Working Paper Series",
 number = "25532",
 year = "2019",
 month = "February",
 doi = {10.3386/w25532},
 URL = "http://www.nber.org/papers/w25532",
 abstract = {},
}


@techreport{Doudchenko16,
 title = "Balancing, Regression, Difference-In-Differences and Synthetic Control Methods: A Synthesis",
 author = "Doudchenko, Nikolay and Imbens, Guido W",
 institution = "National Bureau of Economic Research",
 type = "Working Paper",
 series = "Working Paper Series",
 number = "22791",
 year = "2016",
 month = "October",
 doi = {10.3386/w22791},
 URL = "http://www.nber.org/papers/w22791",
 abstract = {},
}

